Parallel Stochastic Gradient Descent with Sound Combiners

Stochastic gradient descent (SGD) is a well known method for regression and classification tasks. However, it is an inherently sequential algorithm at each step, the processing of the current example depends on the parameters learned from the previous examples. Prior approaches to parallelizing linear learners using SGD, such as HOGWILD! and ALLREDUCE, do not honor these dependencies across threads and thus can potentially suffer poor convergence rates and/or poor scalability. This paper proposes SYMSGD, a parallel SGD algorithm that, to a first-order approximation, retains the sequential semantics of SGD. Each thread learns a local model in addition to a model combiner, which allows local models to be combined to produce the same result as what a sequential SGD would have produced. This paper evaluates SYMSGD's accuracy and performance on 6 datasets on a shared-memory machine shows upto 11x speedup over our heavily optimized sequential baseline on 16 cores and 2.2x, on average, faster than HOGWILD!.

==> back.tex <==
% \section{Outline}
% \label{sec:back}
% \label{sec:outline}
% This section provides the intuitions behind the \ouralgo algorithm
% including the necessary background. The ideas introduced here will be
% formally developed in Section~\ref{sec:algo}.

%\subsection{Regression and Classification}
%Machine learning seeks to explain the relationship of a
%\emph{dependent} variable of interest (say, the house price) to a set
%of \emph{features} (say, the location, the number of bedrooms, etc.)
%by building a parameterized model. The goal then is to determine the
%parameters of the model that minimize some error function on a given
%training dataset. 

%Two of the most common machine learning tasks are linear regression
%and logistic regression. Linear regression predicts the dependent
%variable as a linear function of the features and is useful when the
%variable takes continuous values. Logistic regression learns a
%linear function of the features as well but applies the logistic operator to
%the result to classify the dependent variable into one of two classes.
%Multiclass logistic regression extends this approach to multiple
%classes by learning a linear function per class. 

%\subsection{Stochastic Gradient Descent}
%\label{sec:sgd}
%Stochastic gradient descent (SGD) is a robust method for finding the
%parameters of a model that minimize a given error
%function. This method is popular in searching for the best fitting model
%for linear and logistic regression problems. 
%Figure~\ref{fig:sgdcurve} shows an example of a \emph{convex}
%error function (over two dimensions $x$ and $y$) reaching the minimum
%at parameter $w^*$. Throughout this paper we will assume that error
%function employed is convex, which is indeed the case for linear
%and logistic regressions.


%One approach for finding the optimum $w^*$ is the \emph{batch gradient
%descent} method. Starting from some, not necessarily optimal,
%parameter $w$, this method repeatedly modifies $w$ by taking a step
%along the gradient of the error function at the current $w$.  The
%magnitude of the step is called the learning rate, usually denoted by
%$\alpha$. Computing the gradient requires traversing \emph{every}
%example in the training dataset as each example contributes an error
%term to the total error function. As such, while each step taken by
%this method is accurate, computing the gradient can be expensive for
%large training datasets.

%SGD is a \emph{stochastic} variant of the above method, where the
%gradient is only computed for a randomly chosen example at each
%step. Thus, the gradient computation is efficient but not
%accurate. Nevertheless, SGD enjoys robust convergence
%behavior over large number of steps. This is shown
%pictorially in Figure~\ref{fig:sgdcurve}, where SGD processes examples
%in dataset $D_1$ to reach $w_1$ from $w_g$. During this process, SGD does not
%necessarily move along the true gradient at each step, but does so over
%a large number of steps. 

\section{Background}
% \label{sec:back}
% \label{sec:outline}
%\subsection{Parallelizing Stochastic Gradient Descent}
Stochastic gradient descent (SGD) is a robust method for finding the
parameters of a model that minimize a given error
function. 
%This method is popular in searching for the best fitting model
%for linear and logistic regression problems. 
Figure~\ref{fig:sgdcurve} shows an example of a (convex)
error function over two dimensions $x$ and $y$ reaching the minimum
at parameter $w^*$.
%\footnote{Throughout this paper we will assume that error
%function employed is convex, which is indeed the case for linear
%and logistic regressions.}
\begin{figure}
  \centering
  \includegraphics[width=.5\columnwidth]{figures/ErrorCurve.pdf}
  \caption{Convex error function for a two-dimensional feature space.}
  \label{fig:sgdcurve}
\end{figure}
SGD starts from some, not necessarily optimal,
parameter $w_g$ (as shown in Figure~\ref{fig:sgdcurve}), and repeatedly 
modifies $w$ by taking a step
along the gradient of the error function for a randomly selected example 
at the current $w$. The magnitude of the step is called the learning rate and
is usually denoted by $\alpha$. The gradient computed from one example
is not necessarily the true gradient at $w$. Nevertheless, 
SGD enjoys robust convergence behavior by moving along the ``right''
direction over a large number of steps. This is shown
pictorially in Figure~\ref{fig:sgdcurve}, where SGD processes examples
in dataset $D_1$ to reach $w_1$ from $w_g$.
%During this process, SGD does not
%necessarily move along the true gradient at each step, but does so over
%a large number of steps. 
%SGD is an inherently sequential algorithm. 
%In Figure~\ref{fig:sgdcurve},
%SGD processes a set of examples $D_1$ and moves from $w_g$ to
%$w_1$. 
Subsequently, SGD starts from $w_1$ and processes a different
set $D_2$ to reach $w_h$. There is a clear dependence between
the processing of $D_1$ and the processing of $D_2$ --- the latter
starts from $w_1$, which is only determined after processing $D_1$. 
Our goal is to parallelize SGD despite
this dependence. 

State of the art parallelization techniques such as \hogwild and
\allreduce approach this problem by processing $D_1$ and $D_2$
starting from the same model $w_g$ (let us assume that there only two
processors for now), and respectively reaching $w_1$ and $w_2$. Then,
they combine their local models into a global model, but do so in an
ad-hoc manner. For instance, \allreduce computes a weighted average of
$w_1$ and $w_2$, where the per-feature weights are chosen so as to
prefer the processor that has larger update for that feature. This
weighted average is depicted pictorially as $w_a$. Similarly, in
\hogwild, the two processors race to update the global model with
their respective local model without any locking. (\hogwild performs
this udpate after every example, thus the size of $D_1$ and $D_2$ is
$1$.) Both approaches do not necessarily reach $w_h$, the model that a
sequential SGD would have reached on $D_1$ and $D_2$. While SGD is
algorithmically robust to errors, such ad-hoc combinations can result
in slower convergence (in the case of \allreduce) or poor scalability
across cores(in the case of \hogwild). In contrast, \ouralgo is
significantly faster while maintaing sequential accuracy.

%This paper represents the marriage of a machine learning algorithm
%paper with a systems paper.
We believe \ouralgo generalizes to many forms of distributed hardware,
however, our implementation exploits single-node parallelism. Without
the insights in Section~\ref{sec:impl}, the algorithm is impractical.
We focus on single-node because machine learning is dominated by
single-node installations. At \company\footnote{Anonymized for
  review}, developers trained over 1 million models per month in 2016
on single-node installations. Likewise, Databrick's 2015 survey showed
almost 50\% of Spark installations are single-node~\cite{databricks}.
Modern-shared memory machines have significant resources available to
them---as of September 2016, one can rent an X1 instance from AWS with
2 TB memory and 128 cores for less than \$4 per
hour~\cite{aws-x1-instance} and tens of cores are
commonplace. \ouralgo is ~YYX faster, on average, on this hardware
than prior algorithms which transfers directly to dollars
saved. \note{toddm: replace YYX with actual number}
  

%The \ouralgo algorithm and implementation is designed for
%shared-memory machines. As machines with terabytes of
%memory\footnote{As of September 2016, one can rent an X1 instance from AWS
%with 2 TB memory and 128 cores for less than \$4 per
%hour~\cite{aws-x1-instance}.} and tens of cores are becoming
%commonplace today, scalable shared-memory algorithms can perform
%perform data-intensive machine-learning tasks that would otherwise
%require a distributed solution and associated increase in
%communication costs. 



% % \subsection{Sound Combiner}
% \para{Sound Combiner:}
% The goal of this paper is to 
% \emph{soundly} combine local models. Looking at Figure~\ref{fig:sgdcurve},
% a sound combiner combines local models $w_1$ and $w_2$, respectively
% generated from datasets $D_1$ and $D_2$, into a global model $w_h$
% that is guaranteed to be the same as the model achieved by the
% sequential SGD processing $D_1$ and then $D_2$. In effect, a sound
% combiner allows us to parallelize the sequential computation without
% changing its semantics.

% If we look at the second processor, it starts its computation at
% $w_g$, while in a sequential execution it would have started at $w_1$,
% the output of the first processor. To obtain sequential semantics, we
% need to ``adjust'' its computation from $w_g$ to $w_1$. To do so, the
% second processor performs its computation starting from $w_g + \Delta
% w$, where $\Delta w$ is an \emph{unknown} symbolic vector. This allows
% the second processor to both compute a local model (resulting from the
% concrete part) and a sound combiner (resulting from the symbolic part)
% that accounts for changes in the initial state. Once both processors
% are done learning, second processor finds $w_h$ by setting $\Delta w$
% to $w_1-w_g$ where $w_1$ is computed by the first processor. This
% parallelization approach of SGD can be extended to multiple processors
% where all processor produce a local model and a combiner (except for
% the first processor) and the local models are combined sequentially
% using the combiners.

% When the update to the model parameters is linear in a SGD
% computation, then the dependence on the unknown $\Delta w$ can be
% concisely represented by a \emph{combiner matrix}, as formally described in
% Section~\ref{sec:algo}. Many interesting machine learning algorithms,
% such as linear regression, linear regression with L2 regularization,
% and polynomial regression already have linear update to the
% model parameters (but not necessarily linear on the input
% example). For functions with non-linear updates, a first-order
% approximation still results in a linear dependence. <

% %After the ``learning'' phase, in the ``reduction'' phase, 
% %the second processor computation is
% %shifted by instantiating $\Delta w$ to the difference in start states,
% %$w_1-w_g$. Generalizing this to multiple processors, all except the
% %first processor produce a local model and a combiner matrix. 
% %In the reduction phase, all these local models are combined to generate the same
% %model that the processors would have generated if they had executed
% %sequentially. Of course, this entire process can be iterated to
% %perform multiple SGD steps in parallel. 


% %\subsection{Probabilistically Sound Combiner}
% \para{Probabilistically Sound Combiner:}
% The main problem with generating a sound combiner is that the combiner
% matrix has as many rows and columns as the total number of
% features. Thus, it can be effectively generated only for datasets with
% modest number of features. Most interesting machine learning problems
% involve learning over tens of thousands to billions of features, for
% which maintaining a combiner matrix is clearly not feasible. 

% We solve this problem through dimensionality reduction.
% Johnson-Lindenstrauss~(JL) lemma~\cite{jllemma} allows us to project a set
% of vectors from a high-dimensional space to a random
% low-dimensional space while preserving distances. We use this
% property to reduce the size of the combiner matrix without losing the
% fidelity of the computation---our parallel algorithm produces the
% same result as the sequential SGD in expectation. 

% Of course, a randomized SGD algorithm that generates the exact result
% in expectation is only useful if the resulting variance is small
% enough to maintain accuracy and the rate of convergence. We observe
% that for the variance to be small, the combiner matrix should have
% small singular values. Interestingly, the combiner matrix resulting from
% SGD is dominated by the diagonal entries as the learning rate has to
% be small for effective learning. We use this property to perform the
% JL projection only after {\emph subtracting the identity matrix}. 
% Also, other factors that control the singular values are the learning 
% rate, number of processors, and the frequency of combining local models. 
%Controlling the eigenvalues of the combiner matrix and thus the
%variance of approximation requires careful trade-offs between the ratio
%of computation and communication, which in turn depend on the learning
%rate and the number of processors. 
% This paper explores this design
% space and demonstrates the feasibility of efficient parallelization of
% SGD that retains the convergence properties of sequential SGD while
% enjoying parallel scalability. 



==> motivation.tex <==
%\section{Single-Node Performance}


